Data Driven Validation Framework for Multi-agent Activity-based Models

Activity-based models, as a specific instance of agent-based models, deal with agents that structure their activity in terms of (daily) activity schedules. An activity schedule consists of a sequence of activity instances, each with its assigned start time, duration and location, together with transport modes used for travel between subsequent activity locations. A critical step in the development of simulation models is validation. Despite the growing importance of activity-based models in modelling transport and mobility, there has been so far no work focusing specifically on statistical validation of such models. In this paper, we propose a six-step Validation Framework for Activity-based Models (VALFRAM) that allows exploiting historical real-world data to assess the validity of activity-based models. The framework compares temporal and spatial properties and the structure of activity schedules against real-world travel diaries and origin-destination matrices. We confirm the usefulness of the framework on three real-world activity-based transport models.

==> secActivityBasedModels.tex <==
\section{Multi-agent Activity-based Models}
\mcnote{write this properly. definitions, references and all.\\ }
Agents in activity-based simulation models plan and execute so-called {\em activity schedules} -- finite sequences of {\em activity instances} interconnected by {\em trips}. Each activity instance has a specified {\em type} (e.g. {\tt work}, {\tt school} or {\tt shop}), {\em location}, desired {\em start time} and {\em duration}. Trips between activity instances are specified by their main\footnote{In general, the trips between activities can be multi-modal. In such case, we denote the mode of the longest leg (in terms of travel distance or time) as ``main mode'' and define the whole trip by it.} transport mode (e.g. {\tt car}, {\tt bike} or {\tt public transport}). 

==> secDataSources.tex <==
% content moved to following section
\begin{comment}
\section{Data Sources}\label{sec:data}
A requirement for statistical validation of any model is a data set capturing relevant aspects of the behaviour of reference system, against which the model is validated. It is usually preferable to validate against historical data from real-world systems. However, since such data tends to be difficult or expensive to obtain, models are sometimes validated against data gathered in different models that are known to be valid. This approach, called model alignment, is based on the idea that validity is a transitive relation \cite{axtell1996aligning}.

To validate an activity-based model, VALFRAM framework requires two distinct data sets gathered in the reference system:
\begin{enumerate}
  \item {\em Travel Diaries}: Travel diaries are usually obtained by long-term surveys (taking up to several days), during which participants log all their trips. Resulting data sets contain anonymized information about every participant (usually demographic attributes like age, gender, etc.), and a collection of all their trips with the following properties: {\em time} and {\em date, duration, transport mode(s)} and {\em purpose} (activity type at the destination). More detailed travel diaries also contain the {\em locations} of the origin and destination of each trip.  
  \item {\em Origin-Destination Matrix} (O-D Matrix): The most basic O-D matrices (sometimes called trip tables) are simple two-dimensional square matrices displaying the number trips travelled between every combination of origin and destination locations during specified time period (e.g. one day or one hour). Origin and destination locations are usually predefined, mutually exclusive zones covering the area of interest and their size impacts the level of detail of the matrix. In real-world systems, O-D matrices may be obtained by roadside monitoring, household surveys or derived from global system for mobile communications (GSM) mobile networks \cite{caceres2007deriving}.
\end{enumerate}

Note that similar data sets might in some cases be used during the development of the model (usually when machine learning techniques are involved). However, keep in mind that the same data that was used to build the model should never be used for its validation. 
\end{comment}

